ConFit v2: Improving Resume-Job Matching using Hypothetical Resume Embedding and Runner-Up Hard-Negative Mining

A reliable resume-job matching system helps a company recommend suitable candidates from a pool of resumes and helps a job seeker find relevant jobs from a list of job posts. However, since job seekers apply only to a few jobs, interaction labels in resume-job datasets are sparse. We introduce ConFit v2, an improvement over ConFit to tackle this sparsity problem. We propose two techniques to enhance the encoder's contrastive training process: augmenting job data with hypothetical reference resume generated by a large language model; and creating high-quality hard negatives from unlabeled resume/job pairs using a novel hard-negative mining strategy. We evaluate ConFit v2 on two real-world datasets and demonstrate that it outperforms ConFit and prior methods (including BM25 and OpenAI text-embedding-003), achieving an average absolute improvement of 13.8% in recall and 17.5% in nDCG across job-ranking and resume-ranking tasks.

==> floats/bias.tex <==
\begin{table*}[!t]
\centering
\scalebox{0.6}{
    \begin{tabular}{l cccc}
      \toprule
      & & \multicolumn{4}{c}{\textbf{Intellipro Dataset}} \\
       & \multicolumn{2}{c}{Rank Resume} & \multicolumn{2}{c}{Rank Job} 
    \\
      \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
      \textbf{Model} 
     & nDCG@100 & nDCG@10   \\
      \midrule
      \multirow{1}{*}{V2(w/o gender info)}
    
       &48.17
       &64.91
       \\
      \cmidrule(lr){2-5}
      \multirow{1}{*}{V2(w/ gender info)}
    
       & 49.83
    &67.45

       \\
      \cmidrule(lr){2-5}
      \multirow{1}{*}{V2(w/o gender info)+RUM}
    
         & 50.57
      & 72.38

       \\
      \cmidrule(lr){2-5}
      \multirow{1}{*}{V2(w/ gender info)+RUM}
    
       & 49.76
    &70.16

       \\

   
       
      \bottomrule

    \end{tabular}
  }
\caption{CONFIT bias analysis.}
\label{tbl:bias}
\end{table*}
